Dependences in Strategy Logic

Strategy Logic (SL) is a very expressive logic for specifying and verifying properties of multi-agent systems: in SL, one can quantify over strategies, assign them to agents, and express properties of the resulting plays. Such a powerful framework has two drawbacks: first, model checking SL has non-elementary complexity; second, the exact semantics of SL is rather intricate, and may not correspond to what is expected. In this paper, we focus on strategy dependences in SL, by tracking how existentially-quantified strategies in a formula may (or may not) depend on other strategies selected in the formula. We study different kinds of dependences, refining the approach of [Mogavero et al., Reasoning about strategies: On the model-checking problem, 2014], and prove that they give rise to different satisfaction relations. In the setting where strategies may only depend on what they have observed, we identify a large fragment of SL for which we prove model checking can be performed in 2EXPTIME.

==> app-prop10.tex <==
\EgaleSectionQuatreAuTroisAvril*

\begin{proof}
  The first part can be handle similarly to the first part of Prop~\ref{PropSLCGSideoupasSideRemoveDepende} (Section~\ref{se::Framework} and Annex~\ref{AnnexProposition6::Avril::19}).  
  %
  However, the differentiation are more complex 
  than the ones of Section~\ref{se::Framework}.
  \begin{figure}[b]
    \centering
    \begin{tikzpicture}[xscale=0.9, yscale=0.6]
      \node [draw,rectangle, minimum size=6mm, draw=\FigColB, fill=\FigColB!40!white] (qi) at (0.25,0) {$q$};
      %
      \node [draw,regular polygon, regular polygon sides=5, draw=\FigColD, fill=\FigColD!40!white] (a) at (-2,0) {$a$};
      \node (aA) at (-4.5,+0.75) {$p_1$};
      \node (aB) at (-4.5,-0.75) {$\emptyset$};
      %
      \node [draw,diamond, draw=\FigColC, fill=\FigColC!40!white] (b) at (2,0) {$b$};
      \node [draw, circle, draw=\FigColA, fill=\FigColA!40!white] (c) at (4,0) {$c$};
      \node (cA) at (6,+0.75) {$\emptyset$};
      \node (cB) at (6,-0.75) {$p_2$};
      
      %%%%
      % DRAW
      %%%%
      \draw [-latex'] (qi) to[out=180,in=0] node [above] {\scriptsize $0$} (a);
      \draw [-latex'] (qi) to[out=0,in=180] node [above] {\scriptsize $1$} (b);
      %
      \draw [-latex', rounded corners] (a) to[out=80,in=0] node [text centered, text width=1cm] {\scriptsize $0,0$ \\ $1,1$} (aA);
      \draw [-latex', rounded corners] (a) to[out=-80,in=0] node [text centered, text width=1cm] {\scriptsize $0,1$ \\ $1,0$} (aB);
      %
      \draw [-latex'] (b) to node [text centered, text width=1cm] {\scriptsize $0$ \\ $1$} (c);
      \draw [-latex', rounded corners] (c) to[out=80,in=180] node [text centered, text width=1cm] {\scriptsize $0,0$ \\ $1,1$} (cA);
      \draw [-latex', rounded corners] (c) to[out=-80,in=180] node [text centered, text width=1cm] {\scriptsize $0,1$ \\ $1,0$} (cB);
    \end{tikzpicture}
    \caption{A concurrent game \calG for the proof of Prop.~\ref{Prop-EgaleSection4::3Avril}}
    \label{ConcurrentGameMovingInfoTimelinesChUP}
  \end{figure}
  
  To separate $\models^{\calM(L,T)}$ from $\models^{\calM(L,S,T)}$, consider the game \calG of Fig.~\ref{ConcurrentGameMovingInfoTimelinesChUP} with $6$ agents 
  \BoxFill[\FigColB]{}, \PolygonFill[\FigColD]{1}, \PolygonFill[\FigColD]{2}, \DiamondFill[\FigColC]{}, \CircleFill[\FigColA]{1} and \CircleFill[\FigColA]{2}.
  Each agent can only influence the state represented in its name, for example \CircleFill[\FigColA]{1} and 
  \CircleFill[\FigColA]{2} are the only agents having an influence on the state $c$. To ease the reading we only 
  represented the actions of the active agents on the transitions.
  Consider further the following \SLDG formula
  \begin{alignat*}1
    & \exists x_{p1}^{\BoxUnderFill[\FigColB]{}}.~
    \exists x_{p2}^{\BoxUnderFill[\FigColB]{}}.~
    \exists x^{\CircleUnderFill[\FigColA]{}}_1.~
    \forall x^{\CircleUnderFill[\FigColA]{}}_2.~
    \exists x^{\PolygonUnderFill[\FigColD]{}}_1.~
    \forall x^{\PolygonUnderFill[\FigColD]{}}_2.~
    \exists x^{\DiamondUnderFill[\FigColC]{}}.\
    \\
    &  \bigvee \begin{cases}
      \assign{
	\BoxFill[\FigColB]{}\mapsto x_{p1}^{\BoxUnderFill[\FigColB]{}} ;
	\PolygonFill[\FigColD]{1}\mapsto x^{\PolygonUnderFill[\FigColD]{}}_1; 
	\PolygonFill[\FigColD]{2}\mapsto x^{\PolygonUnderFill[\FigColD]{}}_2; 
	\DiamondFill[\FigColC]{}\mapsto x^{\DiamondUnderFill[\FigColC]{}} ; 
	\CircleFill[\FigColA]{1}\mapsto x^{\CircleUnderFill[\FigColA]{}}_1 ;
	\CircleFill[\FigColA]{2}\mapsto x^{\CircleUnderFill[\FigColA]{}}_2    
      }. \F p_1
      \\
      \assign{
	\BoxFill[\FigColB]{}\mapsto x_{p2}^{\BoxUnderFill[\FigColB]{}} ;
	\PolygonFill[\FigColD]{1}\mapsto x^{\PolygonUnderFill[\FigColD]{}}_1; 
	\PolygonFill[\FigColD]{2}\mapsto x^{\PolygonUnderFill[\FigColD]{}}_2; 
	\DiamondFill[\FigColC]{}\mapsto x^{\DiamondUnderFill[\FigColC]{}} ; 
	\CircleFill[\FigColA]{1}\mapsto x^{\CircleUnderFill[\FigColA]{}}_1 ;
	\CircleFill[\FigColA]{2}\mapsto x^{\CircleUnderFill[\FigColA]{}}_2
      }. \F p_2
    \end{cases}
  \end{alignat*}
  Table~\ref{TableMovingInfoTimelinesChUP} 
  lists the choices of the existential strategies in function of the universal ones and 
  induces a $\calM(L,S,T)$-witness that
  $\calG,q\models^{\calM(L,S,T)} \phi$. On the other hand, 
  Table~\ref{TableMovingInfoTimelinesChUPProngWrong} proves through a case decomposition that 
  $\calG,q\not\models^{\calM(L,T)} \phi$. Both tables can be found in Table~\ref{tab-p10} at the end of this appendix.
  
  The separations for \SLOneG between $\models^{\calM(L,T)}$ and $\models^{\calM(L,F,T)}$, between $\models^{\calM(L,S,T)}$ and $\models^{\calM(L,S,F,T)}$, 
  and between $\models^{\calM(L,F,T)}$ and $\models^{\calM(L,S,F,T)}$ all follow arguments similar to the ones used in Table~\ref{tab-p10} to separate $\models^{\calM(L,T)}$ from $\models^{\calM(L,S,T)}$.
\end{proof}


==> app-prop11.tex <==
\proptimelinesat*

\begin{proof}
  For the cases with \SLCG, consider the game of Fig.~\ref{app-fig-ex} (Annex~\ref{AnnexProposition6::Avril::19}) and the formula~$\phi_C$ below.
  For the cases with \SLDG, take the game of Fig.~\ref{app-fig-exbis} (Annex~\ref{AnnexProposition6::Avril::19}) and the formula~$\phi_D$ below. 
  The verification is similar to many result done before.
  
  \begin{alignat*}1
    \phi_C &=\exists y.\ \forall x_A.\ \exists x_B .\
    \bigwedge
    \begin{cases}
      \assign{\CircleFill[\FigColA]{}\mapsto y;\ \BoxFill[\FigColB]{}\mapsto x_A}.\  \F p_1 \
      \\
      \assign{\CircleFill[\FigColA]{}\mapsto y;\ \BoxFill[\FigColB]{}\mapsto x_B}.\  \F p_2
    \end{cases}
    \\
    \phi_D &=\exists y.\ \forall x_A.\ \forall x_B.\ \forall z.\
    \bigvee
    \begin{cases} 
      \assign{\CircleFill[\FigColA]{}\mapsto  y ; \BoxFill[\FigColB]{}\mapsto  x_A ; \DiamondFill[\FigColC]{} \mapsto z}.\ \F p_1 
      \\
      \assign{\CircleFill[\FigColA]{}\mapsto  y ; \BoxFill[\FigColB]{}\mapsto  x_B ; \DiamondFill[\FigColC]{} \mapsto z}.\ \F p_2  
    \end{cases}
  \end{alignat*}
\end{proof}


==> app-prop3.tex <==
\PropositionTroisAvril*


\begin{proof}
  In the paper, we proved the result for $\models^{\calM(L)}$.  The
  remaining two cases can be handled similarly.  The counter-example
  for $\models^{\calM(L,F)}$ uses the game on the left of
  Fig.~\ref{3::Mars::2017::CanNeitherHold::Chap5::FIGURE:::2::Lemaas}
  and the following formula
  \[
  \phi =\forall x.\ \exists y.\ \bigwedge
  \begin{cases}
    \assign{\CircleFill[\FigColA]{}\mapsto x}.\ \F
       p_1 \Leftrightarrow \assign{\CircleFill[\FigColA]{}\mapsto y}.\ \F p_1
    \\
    \assign{\CircleFill[\FigColA]{}\mapsto x}.\ \F p_2
       \Leftrightarrow \assign{\CircleFill[\FigColA]{}\mapsto y}.\ \F p_2
  \end{cases}
  \]
  %
  Checking that both $\phi$ and $\neg\phi$ fail to hold follows
  similar arguments to the ones used in the paper for
  $\models^{\calM(L)}$.  The counter-example for
  $\models^{\calM(L,S)}$ uses the game to the right of
  Fig.~\ref{3::Mars::2017::CanNeitherHold::Chap5::FIGURE:::2::Lemaas}
  and the formula $ \phi=\forall x.\ \exists y.\ \bigl(
  \assign{\CircleFill[\FigColA]{}\mapsto x}.\ \F p_1 \Leftrightarrow
  \assign{\CircleFill[\FigColA]{}\mapsto y}.\ \F p_2 \bigr)$.
\end{proof}
\begin{figure}[ht]
  \centering
  \begin{tikzpicture}
    \node [circle, draw, fill=\FigColA!40!white] (qinit) at (0,0) {$q_0$};
    \node [circle, draw, fill=\FigColA!40!white] (a) at (-1.5,-1) {$A$}; \node (p1) at (-1.5-0.75,-2) {$p_1$}; \node (p2) at (-1.5+0.75,-2) {$p_2$};
    \node [circle, draw, fill=\FigColA!40!white] (b) at (1.5,-1) {$B$}; \node (p3) at (1.5-0.75,-2) {$p_1$}; \node (p4) at (1.5+0.75,-2) {$p_2$};
    %
    \draw[-latex'] (qinit) to (a); \draw[-latex'] (qinit) to (b);
    \draw[-latex'] (a) to (p1);\draw[-latex'] (a) to (p2);
    \draw[-latex'] (b) to (p3);\draw[-latex'] (b) to (p4);
  \end{tikzpicture}
  ~\qquad ~
  \begin{tikzpicture}
    \node [circle, draw, fill=\FigColA!40!white] (qinit) at (0,0) {$q_0$};
    \node [circle, draw, fill=\FigColA!40!white] (a) at (-1.5,-1) {$A$}; \node (p1) at (-1.5-0.75,-2) {$p_1$}; \node (p2) at (-1.5+0.75,-2) {$\emptyset$};
    \node [circle, draw, fill=\FigColA!40!white] (b) at (1.5,-1) {$p_2$}; 
    %
    \draw[-latex'] (qinit) to (a); \draw[-latex'] (qinit) to (b);
    \draw[-latex'] (a) to (p1);\draw[-latex'] (a) to (p2);
  \end{tikzpicture}
  \caption{Two games for the proof of Prop.~\ref{Chapitre3Framework::Prop::NeitherHold::31MArs2017}.}
  \label{3::Mars::2017::CanNeitherHold::Chap5::FIGURE:::2::Lemaas}
\end{figure}



==> app-tables.tex <==
    \begin{sidewaystable}
      \centering
      \begin{tikzpicture}[xscale=0.8]
	% LIGNE DES NOEUDS
	\node (x2) at (0,1) {$x_2(q_3)$}; \node (x2) at (0,0.5) {$x_4(q_3)$}; \node (x5) at (0,0) {$x_5(q_3)$}; %forall
	\node (x1) at (2,1) {$x_1(q_3)$}; \node (x3) at (2,0.5) {$x_3(q_3)$}; \node (x6) at (2,0) {$x_6(q_3)$}; %exists
	\node (z1) at (4,0.75) {$z_1(q_3.A)$}; \node (y1) at (4,0.25) {$y_1(q_3.A.C)$}; %exists
	\node (v5) at (6,0.5) {$v_5(q_3.D)$}; %forall
	\node (v6) at (8,0.5) {$v_6(q_3.D)$}; %exists
	\node (w2) at (10,0.5) {$w_2(q_3.B)$}; %forall
	\node (w3) at (12,0.5) {$w_3(q_3.B)$}; %exists
	\node (z4) at (14,0.5) {$z_4(q_3.A)$}; %forall
	%      
	\draw (-1,-0.25) rectangle (21+1,1.25);
	\draw (-1,-0.22) to (21+1,-0.22);
	% LIGNE DES QUANTIFICATIONS        
	\draw (-1,1.25) rectangle (1,1.75); \node at (0,1.5) {$\forall$};
	\draw (1,1.25) rectangle (5,1.75); \node at (3,1.5) {$\exists$};
	\draw (5,1.25) rectangle (7,1.75); \node at (6,1.5) {$\forall$};
	\draw (7,1.25) rectangle (9,1.75); \node at (8,1.5) {$\exists$};
	\draw (9,1.25) rectangle (11,1.75); \node at (10,1.5) {$\forall$};
	\draw (11,1.25) rectangle (13,1.75); \node at (12,1.5) {$\exists$};
	\draw (13,1.25) rectangle (15,1.75); \node at (14,1.5) {$\forall$};
	%%%%%%%%%%%%%
	%% Debut des lignes
	%%%%%%%%%%%%%
	% PREMIER BLOC
	\node at (0,-0.75) {\small \begin{tabular}{c}$\star,\star,A$\\ or~$\star,\star,B$\end{tabular}};
	\node at (2,-0.75) {\small $A,\star,\star$};
	\node at (4,-0.75) {\small $C,\emptyset$};
	\node at (17.5+0.75,-0.75) {\small $\neg\psi_1,\neg \psi_5$};
	\draw (-1,-0.25) rectangle (21+1,-1.25);
	% DEUXIEME BLOC
	\node at (0,-1.75) {\small $A,\star,D$};
	\node at (2,-1.75) {\small $A,A,D$};
	\node at (4,-1.75) {\small $C,p_1$};
	\node at (6,-1.5) {\small $p_5$}; \node at (8,-1.5) {\small $p_6$};
	\node at (6,-2) {\small $p_6$}; \node at (8,-2) {\small $p_5$};
	\node at (17.5+0.75,-1.5) {\small $\psi_1,\psi_5$};
	\node at (17.5+0.75,-2) {\small $\psi_1,\neg\psi_2,\neg\psi_3, \neg \psi_5 ,\neg\psi_6$ (OK no matter $\psi_4$)};
	\draw (-1,-1.25) rectangle (21+1,-2.25);
	% TROISIEME BLOC
	\node at (0,-3.25) {\small $B,B,D$};
	\node at (2,-3.25) {\small $B,B,D$};
	\node at (6,-2.5) {\small $p_5$}; \node at (8,-2.5) {\small $p_6$};
	\node at (6,-3) {\small $p_5$}; \node at (8,-3) {\small $p_6$};
	\node at (6,-3.5) {\small $p_6$}; \node at (8,-3.5) {\small $p_5$};
	\node at (6,-4) {\small $p_6$}; \node at (8,-4) {\small $p_5$};
	\node at (10,-2.5) {\small $p_2$}; \node at (12,-2.5) {\small $p_3$};
	\node at (10,-3) {\small $p_3$}; \node at (12,-3) {\small $p_2$};
	\node at (10,-3.5) {\small $p_2$}; \node at (12,-3.5) {\small $p_3$};
	\node at (10,-4) {\small $p_3$}; \node at (12,-4) {\small $p_2$};
	\node at (14,-5.25) {$p_4$};
	\node at (17.5+0.75,-2.5) {\small $\neg \psi_1,\psi_2,\psi_3,\neg\psi_4,\psi_5 ,\psi_6$};
	\node at (17.5+0.75,-3) {\small $\neg \psi_1,\neg \psi_2,\neg \psi_3,\neg\psi_4,\psi_5 ,\psi_6$}; 
	\node at (17.5+0.75,-3.5) {\small $\neg \psi_1,\psi_2,\psi_3,\neg\psi_4,\neg\psi_5 ,\neg\psi_6$}; 
	\node at (17.5+0.75,-4) {\small $\neg \psi_1,\neg\psi_2,\neg\psi_3,\neg\psi_4,\neg\psi_5 ,\neg\psi_6$}; 
	
	\draw (-1,-4.25) rectangle (21+1,-2.25);
	% QUATRIEME BLOC
	\node at (0,-5.25) {\small $B,A,D$};
	\node at (2,-5.25) {\small $A,B,D$};
	\node at (4,-5.25) {\small $C,\ p_1$};
	\node at (6,-4.5) {\small $p_5$}; \node at (8,-4.5) {\small $p_6$};
	\node at (6,-5) {\small $p_5$}; \node at (8,-5) {\small $p_6$};
	\node at (6,-5.5) {\small $p_6$}; \node at (8,-5.5) {\small $p_5$};
	\node at (6,-6) {\small $p_6$}; \node at (8,-6) {\small $p_5$};
	\node at (10,-4.5) {\small $p_2$}; \node at (12,-4.5) {\small $p_3$};
	\node at (10,-5) {\small $p_3$}; \node at (12,-5) {\small $p_2$};
	\node at (10,-5.5) {\small $p_2$}; \node at (12,-5.5) {\small $p_3$};
	\node at (10,-6) {\small $p_3$}; \node at (12,-6) {\small $p_2$};
	\node at (17.5+0.75,-4.5) {\small $\psi_1,\psi_2,\psi_3,\psi_4,\psi_5 ,\psi_6$};
	\node at (17.5+0.75,-5) {\small $\psi_1,\neg \psi_2,\neg \psi_3,\psi_4,\psi_5 ,\psi_6$}; 
	\node at (17.5+0.75,-5.5) {\small $\psi_1,\psi_2,\psi_3,\psi_4,\neg\psi_5 ,\neg\psi_6$}; 
	\node at (17.5+0.75,-6) {\small $\psi_1,\neg\psi_2,\neg\psi_3,\psi_4,\neg\psi_5 ,\neg\psi_6$}; 
	\draw (-1,-4.25) rectangle (21+1,-6.25);
	% CINQUIEME BLOC
	\node at (0,-7.25) {\small $B,A,D$};
	\node at (2,-7.25) {\small $A,B,D$};
	\node at (4,-7.25) {\small $C,\ \emptyset$};
	\node at (6,-6.5) {\small $p_5$}; \node at (8,-6.5) {\small $p_6$};
	\node at (6,-7) {\small $p_5$}; \node at (8,-7) {\small $p_6$};
	\node at (6,-7.5) {\small $p_6$}; \node at (8,-7.5) {\small $p_5$};
	\node at (6,-8) {\small $p_6$}; \node at (8,-8) {\small $p_5$};
	\node at (10,-6.5) {\small $p_2$}; \node at (12,-6.5) {\small $p_3$};
	\node at (10,-7) {\small $p_3$}; \node at (12,-7) {\small $p_2$};
	\node at (10,-7.5) {\small $p_2$}; \node at (12,-7.5) {\small $p_3$};
	\node at (10,-8) {\small $p_3$}; \node at (12,-8) {\small $p_2$};  
	\node at (14,-7.25) {$C$};
	\node at (17.5+0.75,-6.5) {\small $\neg \psi_1,\psi_2,\psi_3,\neg\psi_4,\psi_5 ,\psi_6$};
	\node at (17.5+0.75,-7) {\small $\neg \psi_1,\neg \psi_2,\neg \psi_3,\neg \psi_4,\psi_5 ,\psi_6$}; 
	\node at (17.5+0.75,-7.5) {\small $\neg \psi_1,\psi_2,\psi_3,\neg\psi_4,\neg\psi_5 ,\neg\psi_6$}; 
	\node at (17.5+0.75,-8) {\small $\neg \psi_1,\neg\psi_2,\neg\psi_3,\neg\psi_4,\neg\psi_5 ,\neg\psi_6$}; 
	\draw (-1,-8.25) rectangle (21+1,-6.25);
	%%%%%%%%%%%%%%%%%%%%
	%%   DEPENDENCES
	%%%%%%%%%%%%%%%%%%%%
	\draw[decoration={brace,mirror,raise=9pt},decorate, red]
	(-0.9,-8) -- (0.9,-8);
	\draw[decoration={brace,mirror,raise=9pt},decorate, red]
	(1.1,-8) -- (4.9,-8);
	\draw [bend right=20,->, red] (0,-8.5) to node[red,fill=white] {$local$} (3,-8.5);
	%%%%%%%%%%%%%%%%%%%%
	\draw[decoration={brace,mirror,raise=9pt},decorate, red]
	(5.1,-8) -- (6.9,-8);
	\draw[decoration={brace,mirror,raise=9pt},decorate, red]
	(7.1,-8) -- (8.9,-8);
	\draw [bend right=20,->, red] (6,-8.5) to node[red, fill=white] {$local$} (8,-8.5);
	%%%%%%%%%%%%%%%%%%%%
	\draw[decoration={brace,mirror,raise=9pt},decorate, red]
	(5.1+4,-8) -- (6.9+4,-8);
	\draw[decoration={brace,mirror,raise=9pt},decorate, red]
	(7.1+4,-8) -- (8.9+4,-8);
	\draw [bend right=20,->, red] (6+4,-8.5) to node[red, fill=white] {$local$} (8+4,-8.5);
	%%%%%%%%%%%%%%%%%%%%
	\draw [red, thick, dashed] (4.25,-5.25) circle (0.3cm);
	\draw [red, thick, dashed] (4.25,-7.25) circle (0.3cm);
	\draw [red, thick, dashed] (14,-5.25) circle (0.3cm);
	\draw [red, thick, dashed] (14,-7.25) circle (0.3cm);
	\draw [->, dashed ,red, thick] (14,-4.8) to[out=45+90,in=0] (4.25,-4.8);
	\node [red, fill=white] at (13.8,-4) {\small Unordered Prefix};
	\draw [->, dashed ,red, thick] (14,-6.8) to[out=45+90,in=0] (4.25,-6.8);
	\node [red, fill=white] at (13.8,-6) {\small Unordered Prefix};
      \end{tikzpicture}
      \caption{Table for the proof of Proposition~\ref{PropNegationsAndCo::DeuxTroisAvril::ccr:::deux}.}
      \label{FigureTablesidewayLemmaNegationProbLSEPmap}
    \end{sidewaystable}
    
    
    
    \begin{sidewaystable}
      \centering
      \begin{tikzpicture}[yscale=1.2]
	% LIGNE DES NOEUDS
	\node (x2) at (0,1) {\small $x_2(q_3)$}; \node (x2) at (0,0.5) {\small $x_4(q_3)$}; \node (x5) at (0,0) {\small $x_5(q_3)$}; %forall
	\node (x1) at (2,1) {\small $x_1(q_3)$}; \node (x3) at (2,0.5) {\small $x_3(q_3)$}; \node (x6) at (2,0) {\small $x_6(q_3)$}; %exists
	\node (z1) at (4,0.25) {\small $z_1(q_3.A)$}; \node (y1) at (4,0.75) {\small $y_1(q_3.A.C)$}; %exists
	\node (v5) at (6,0.5) {\small $v_5(q_3.D)$}; %forall
	\node (v6) at (8,0.5) {\small $v_6(q_3.D)$}; %exists
	\node (w2) at (10,0.5) {\small $w_2(q_3.B)$}; %forall
	\node (w3) at (12,0.5) {\small $w_3(q_3.B)$}; %exists
	\node (z4) at (14,0.5) {\small $z_4(q_3.A)$}; %forall
	%      
	\draw (-1,-0.25) rectangle (21+1,1.25);
	\draw (-1,-0.22) to (21+1,-0.22);
	% LIGNE DES QUANTIFICATIONS        
	\draw (-1,1.25) rectangle (1,1.75); \node at (0,1.5) {$\exists$};
	\draw (1,1.25) rectangle (5,1.75); \node at (3,1.5) {$\forall$};
	\draw (5,1.25) rectangle (7,1.75); \node at (6,1.5) {$\exists$};
	\draw (7,1.25) rectangle (9,1.75); \node at (8,1.5) {$\forall$};
	\draw (9,1.25) rectangle (11,1.75); \node at (10,1.5) {$\exists$};
	\draw (11,1.25) rectangle (13,1.75); \node at (12,1.5) {$\forall$};
	\draw (13,1.25) rectangle (15,1.75); \node at (14,1.5) {$\exists$};
	%%%%%%%%%%%%%
	%% Debut des lignes 
	%%%%%%%%%%%%%
	% PREMIER BLOC
	\node at (0,-1) {\scriptsize $B,A,D$};
	\node at (2,-1) {\scriptsize $\star,A,\star$ or $\star,D,\star$};
	\node at (10,-1) {\scriptsize $p_2$};
	\node at (4,-0.5) {\scriptsize $p_4,\star$};
	\node at (4,-1) {\scriptsize $C,\emptyset$};
	\node at (4,-1.5) {\scriptsize $C,p_1$};
	\node at (6,-0.5) {\scriptsize $p_5$};
	\node at (6,-1) {\scriptsize $p_5$};
	\node at (6,-1.5) {\scriptsize $p_6$};
	\node at (17.5,-0.5) {\scriptsize $\neg \psi_1,\psi_2,\neg \psi_3,\psi_5$};
	\node at (17.5,-1) {\scriptsize $\neg\psi_1,\psi_2,\neg \psi_3,\psi_5$};
	\node at (17.5,-1.5) {\scriptsize $\psi_1,\psi_2,\neg \psi_3,\neg\psi_5$};
	%
	\draw (-1,-0.25) rectangle (21+1,-1.75);
	
	% DEUXIEME BLOC
	\node at (0,-2) {\scriptsize $B,A,D$};
	\node at (2,-2) {\scriptsize $B,B,\star$};
	\node at (6,-2) {\scriptsize $p_5$};	 
	\node at (10,-2) {\scriptsize $p_3$};
	\node at (14,-2) {\scriptsize $p_4$};	
	\node at (17.5,-2) {\scriptsize $\neg \psi_1,\neg \psi_2,\psi_4,\psi_5$};
	%
	\draw (-1,-0.25) rectangle (21+1,-2.25);
	
	% Troisieme bloc
	\node at (0,-2.75) {\scriptsize $B,A,D$};
	\node at (2,-2.75) {\scriptsize $A,B,A$ or $A,B,B$};
	%
	\node at (4,-2.5) {\scriptsize $p_4,\star$ or $C,\emptyset$};
	\node at (6,-2.5) {\scriptsize $p_5$};
	\node at (17.5,-2.5) {\scriptsize $\neg\psi_1,\psi_5,\neg \psi_6$};
	%
	\node at (4,-3) {\scriptsize $C,p_1$};
	\node at (6,-3) {\scriptsize $p_6$};
	\node at (10,-3) {\scriptsize $p_2$};
	\node at (14,-3) {\scriptsize $C$};
	\node at (17.5,-3) {\scriptsize $\psi_1,\psi_2, \neg \psi_4, \neg \psi_5,\neg\psi_6$ (OK no matter $\psi_3$)};
	%
	\draw (-1,-0.25) rectangle (21+1,-3.25);
	
	
	
	% Quatrieme BLOC
	\node at (0,-3.5) {\scriptsize $B,A,D$};
	\node at (2,-3.5) {\scriptsize $A,B,D$};
	\node at (4,-3.5) {\scriptsize $p_4,\star$ or $C,\emptyset$};
	\node at (6,-3.5) {\scriptsize $p_5$};	 
	%
	\draw [thin, opacity=0.5] (-0.5,-3.75) to (20.5,-3.75);
	%	
	\node at (8,-4) {\scriptsize $p_5$};
	\node at (17.5,-4) {\scriptsize $\neg \psi_1,\psi_5,\neg \psi_6$};
	%
	\node at (8,-4.5) {\scriptsize $p_6$};
	\node at (10,-4.5) {\scriptsize $p_3$};
	\node at (14,-4.5) {\scriptsize $p_4$};
	\node at (17.5,-4.5) {\scriptsize $\neg \psi_1,\neg\psi_2,\psi_4,\psi_5,\psi_6$ (OK no matter $\psi_3$)};
	% 
	\draw (-1,-0.25) rectangle (21+1,-4.75);
	
	% cinq BLOC
	\node at (0,-5) {\scriptsize $B,A,D$};
	\node at (2,-5) {\scriptsize $A,B,D$};
	\node at (4,-5) {\scriptsize$C,p_1$};	
	\node at (6,-5) {\scriptsize $p_6$};	 
	% 	%
	\draw [thin, opacity=0.5] (-0.5,-5.25) to (20.5,-5.25);
	% 	%
	\node at (8,-5.5) {\scriptsize $p_6$};
	\node at (17.5,-5.5) {\scriptsize $\psi_1,\neg\psi_5,\psi_6$};
	% 	%
	\node at (8,-6) {\scriptsize $p_5$};
	\node at (10,-6) {\scriptsize $p_2$};
	\node at (14,-6) {\scriptsize $C$};
	\node at (17.5,-6) {\scriptsize $\psi_1,\psi_2,\neg\psi_4,\neg\psi_5,\neg\psi_6$ (OK no matter $\psi_3$)};
	% 	%
	\draw (-1,-0.25) rectangle (21+1,-6.25);
	%%%%%%%%%%%%%%%%%
	%% DEPENDENCES
	%%%%%%%%%%%%%%%%%
	\draw[decoration={brace,mirror,raise=9pt},decorate, red] (1,-6.2) -- (5,-6.2);
	\draw[decoration={brace,mirror,raise=9pt},decorate, red] (5,-6.2) -- (7,-6.2);
	\draw[decoration={brace,mirror,raise=9pt},decorate, red] (7,-6.2) -- (9,-6.2);
	\draw[decoration={brace,mirror,raise=9pt},decorate, red] (9,-6.2) -- (11,-6.2);
	%
	\draw [->, red] (3,-6.5-0.2) to[out=-40, in=-90-45] node[red, fill=white, ] {\scriptsize local$+$side} (10,-6.5-0.2);
	\draw [bend right=20,->, red] (8,-6.5-0.2) to node[red, fill=white, ] {\scriptsize side} (10,-6.5-0.2);
	\draw [bend right=20,->, red] (3,-6.5-0.2) to node[red, fill=white, ] {\scriptsize local$+$side} (6,-6.5-0.2);
	%
	%
	\draw [red, thick, dashed] (14,-2) circle (0.3cm);
	\draw [red, thick, dashed] (2-0.5,-2-0.25) rectangle (2+0.5,-2+0.25);
	\draw [-, dashed ,red, thick] (14,-1.65) to[out=55+90,in=0] node [text=red, fill=white] {\scriptsize local} (2,-1.75);
	%
	\draw [red, thick, dashed] (14,-3) circle (0.3cm);
	\draw [red, thick, dashed] (2-1.2,-2.75-0.2) rectangle (2+1.2,-2.75+0.2);
	\draw [-, dashed ,red, thick] (14,-3+0.3+0.05) to[out=90+55,in=0] node [text=red, fill=white] {\scriptsize local} (2+1.2,-2.75);
	%
	\draw [red, thick, dashed] (14,-4.5) circle (0.3cm);
	\draw [red, thick, dashed] (8,-4.5) circle (0.3cm);
	\draw [red, thick, dashed] (2+0.6,-3.5+0.25) rectangle (2-0.6,-3.5-0.25);
	\draw [-, dashed ,red, thick] (14,-4.5+0.35) to[out=90+55,in=-40] node [text=red, fill=white] {\scriptsize local} (2+0.6,-3.5);
	\draw [-, dashed ,red, thick] (14,-4.5+0.35) to[out=90+55,in=0] node [text=red, fill=white] {\scriptsize side} (8+0.3,-4.5);
	
	%
	\draw [red, thick, dashed] (14,-6) circle (0.3cm);
	\draw [red, thick, dashed] (8,-6) circle (0.3cm);
	\draw [red, thick, dashed] (2+0.6,-5+0.25) rectangle (2-0.6,-5-0.25);	
	\draw [-, dashed ,red, thick] (14,-6+0.35) to[out=90+55,in=-40] node [text=red, fill=white] {\scriptsize local} (2+0.6,-5);
	\draw [-, dashed ,red, thick] (14,-6+0.35) to[out=90+55,in=0] node [text=red, fill=white] {\scriptsize side} (8+0.3,-6);
	
      \end{tikzpicture}
      \caption{Second table for the proof of Prop.~\ref{PropNegationsAndCo::DeuxTroisAvril::ccr:::deux}.}
      \label{FigureTablesidewayLemmaNegationProbLSEPmapBIS}
    \end{sidewaystable}
    
    
    \begin{sidewaystable} 
      \begin{subtable}{\textwidth}
	\centering
	\begin{tabular}{cc|cccc|c}
	  \multirow{2}{*}{$w$}
	  & $x^{\CircleUnderFill[\FigColA]{}}_2$ & $0$ & $0$ 
	  & $1$ & $1$ &
	  \\
	  & $x^{\PolygonUnderFill[\FigColD]{}}_2$ & $0$  & $1$
	  & $0$ & $1$ & 
	  \\ 
	  \hline 
	  %
	  \multirow{5}{*}{$\theta(w)$}
	  & $x_{p1}^{\BoxUnderFill[\FigColB]{}}$ & $0$ & $0$ & $0$ & $0$ 
	  & Depend on nothing
	  \\
	  & $x_{p2}^{\BoxUnderFill[\FigColB]{}}$ & $1$ & $1$ & $1$ & $1$ 
	  & Depend on nothing
	  \\
	  & $x^{\DiamondUnderFill[\FigColC]{}}$ & $0$ & $1$ 
	  & $0$ & $1$ 
	  & Depend on $x_{p1}^{\BoxUnderFill[\FigColB]{}}$, $x_{p2}^{\BoxUnderFill[\FigColB]{}}$ and $x^{\PolygonUnderFill[\FigColD]{}}_2$
	  ($x^{\DiamondUnderFill[\FigColC]{}}=x^{\PolygonUnderFill[\FigColD]{}}_2$)
	  \\
	  & $x^{\CircleUnderFill[\FigColA]{}}_1$ & $0$ & $1$
	  & $0$ & $1$ 
	  & Depend on $x_{p1}^{\BoxUnderFill[\FigColB]{}}$, $x_{p2}^{\BoxUnderFill[\FigColB]{}} $ and $x^{\DiamondUnderFill[\FigColC]{}}$
	  ($x^{\CircleUnderFill[\FigColA]{}}_1=x^{\DiamondUnderFill[\FigColC]{}}$)
	  \\
	  & $x^{\PolygonUnderFill[\FigColD]{}}_1$ & $0$ & $0$
	  & $1$ & $1$ 
	  &  Depend on $x_{p1}^{\BoxUnderFill[\FigColB]{}}$, $x_{p2}^{\BoxUnderFill[\FigColB]{}}$, $x^{\DiamondUnderFill[\FigColC]{}}$ and $x^{\CircleUnderFill[\FigColA]{}}_2$
	  ($x^{\PolygonUnderFill[\FigColD]{}}_1=x^{\CircleUnderFill[\FigColA]{}}_2$)
	  \\
	  \hline
	  \multirow{2}{*}{result}
	  & Goal 1 & ok & no & no & ok
	  \\
	  & Goal 2 & no & ok & ok & no
	\end{tabular}
	\caption{Building the map $\theta$ to prove $\calG,q\models^{\calM(L,S,T)}$ in Proposition~\ref{Prop-EgaleSection4::3Avril}.}
	\label{TableMovingInfoTimelinesChUP}
      \end{subtable}
      ~$\newline$
      ~$\newline$
      \begin{subtable}{\textwidth}
	\centering
	\begin{tabular}{cc|c|c|c|c|c}
	  & 
	  & \multicolumn{2}{c|}{if $x_{p2}^{\BoxUnderFill[\FigColB]{}} = 0$}  
	  & \multicolumn{2}{c|}{if $x_{p1}^{\BoxUnderFill[\FigColB]{}} = 1$} 
	  & if $x_{p1}^{\BoxUnderFill[\FigColB]{}} = 0$ and $x_{p2}^{\BoxUnderFill[\FigColB]{}} = 1$
	  \\
	  & 
	  & if ($x^{\PolygonUnderFill[\FigColD]{}}_1 = 0$) & if ($x^{\PolygonUnderFill[\FigColD]{}}_1 = 1$)
	  & if ($x^{\CircleUnderFill[\FigColA]{}}_1 = 0$) & if ($x^{\CircleUnderFill[\FigColA]{}}_1 = 1$)
	  & Case with $x^{\PolygonUnderFill[\FigColD]{}}_1 = 0$ and $x^{\CircleUnderFill[\FigColA]{}}_1 = 0$ ; other cases are similar
	  \\
	  \hline
	  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	  \multirow{2}{*}{$w$} & $x^{\CircleUnderFill[\FigColA]{}}_2$ 
	  & - & -
	  & $0$ & $1$
	  & $0$
	  \\
	  & $x^{\PolygonUnderFill[\FigColD]{}}_2$
	  & $1$ & $0$
	  & - & -
	  & $1$
	  \\
	  \hline
	  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	  \multirow{4}{*}{$\theta(w)$} & $x_{p1}^{\BoxUnderFill[\FigColB]{}}$
	  & - & -
	  & $1$ & $1$ 
	  & $0$
	  \\
	  & $x_{p2}^{\BoxUnderFill[\FigColB]{}}$
	  & $0$ & $0$
	  & - & -
	  & $1$
	  \\
	  & $x^{\DiamondUnderFill[\FigColC]{}}$
	  & - & -
	  & - & -
	  & -
	  \\ 
	  & $x^{\PolygonUnderFill[\FigColD]{}}_1$
	  & $0$ & $1$
	  & - & -
	  & $0$
	  \\
	  & $x^{\CircleUnderFill[\FigColA]{}}_1$
	  & - & -
	  & $0$ & $1$
	  & $0$
	  \\
	  \hline
	  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	  \multirow{4}{*}{result} & \multirow{2}{*}{Goal~1}
	  & $q.a.\emptyset$ & $q.a.\emptyset$
	  & $q.b.c.\emptyset$ & $q.b.c.\emptyset$ 
	  & $q.a.\emptyset$
	  \\
	  & 
	  & no & no
	  & no & no
	  & no
	  \\
	  \cline{3-7}
	  %
	  & \multirow{2}{*}{Goal~2}
	  & $q.a.\emptyset$ & $q.a.\emptyset$
	  & $q.b.c.\emptyset$ & $q.b.c.\emptyset$ 
	  & $q.b.c.\emptyset$
	  \\
	  &
	  & no & no
	  & no & no
	  & no
	\end{tabular}
	
	\caption{Proving $\calG,q\not\models^{\calM(L,T)}$ in Prop.~\ref{Prop-EgaleSection4::3Avril}.}
	\label{TableMovingInfoTimelinesChUPProngWrong}
      \end{subtable}
      \caption{Tables for Proposition~\ref{Prop-EgaleSection4::3Avril}.}
      \label{tab-p10}
    \end{sidewaystable}


==> fig-lsf.tex <==
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[xscale=1, yscale=0.7]
    \begin{scope}
    \node [circle, draw, scale =0.7] (a) at (0,0) {$\forall  x_1$}; 
    \node [text width=2.1cm] at (-1.25+0.05,-0.5) {\scriptsize \begin{tabular}{c}Local \\dependences\\(always \\allowed)\end{tabular}}; 
    \draw [-latex'] (a) to (-1.4,-3);
    \draw [-latex'] (a) to (1.4,-3);
    \node [draw, scale=0.8] (aa) at (-0.25,-1.5) {};
    \node [draw, scale=0.8] (aaa) at (-0.8,-2.5) {};
    \node[below=1pt] at (aaa) {$p$};
    \node [draw, scale=0.8] (aaaa) at (-0.3,-2.5) {};
    \node [draw, scale=0.8] (paa) at (0.25,-1.5) {};
    \node [draw, scale=0.8] (paaa) at (0.8,-2.5) {};
    \node [draw, scale=0.8] (paaaa) at (0.3,-2.5) {};
    \node[below=1pt] at (paaaa) {$q$};
    \draw [-latex', opacity=0.35] (a) to (aa);
    \draw [-latex', opacity=0.35] (aa) to (aaa);
    \draw [-latex',  opacity=0.35] (aa) to (aaaa);
    \draw [-latex', opacity=0.35] (a) to (paa);
    \draw [-latex', opacity=0.35] (paa) to (paaa);
    \draw [-latex',  opacity=0.35] (paa) to (paaaa);
    
    \node [scale =0.7, circle, draw] (b) at (3,0) {$\exists  x_2$};
    \draw [-latex'] (b) to (-1.4+3,-3);
    \draw [-latex'] (b) to (1.4+3,-3);
    \node [draw, scale=0.8] (bb) at (-0.25+3,-1.5) {};
    \node [draw, scale=0.8] (bbb) at (-0.8+3,-2.5) {};
    \node[below=1pt] at (bbb) {$p$};
    \node [draw, scale=0.8] (bbbb) at (-0.3+3,-2.5) {};
    \node [draw, scale=0.8] (pbb) at (0.25+3,-1.5) {};
    \node [draw, scale=0.8] (pbbb) at (0.8+3,-2.5) {};
    \node [draw, scale=0.8] (pbbbb) at (0.3+3,-2.5) {};
    \node[below=1pt] at (pbbbb) {$q$};
    \draw [-latex', opacity=0.35] (b) to (bb);
    \draw [-latex',  opacity=0.35] (bb) to (bbb);
    \draw [-latex',  opacity=0.35] (bb) to (bbbb);
    \draw [-latex', opacity=0.35] (b) to (pbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbbb);
    
    \node [circle,draw, scale =0.7] (c) at (6,0) {$\forall x_3$}; 
    \draw [-latex'] (c) to (-1.4+6,-3);
    \draw [-latex'] (c) to (1.4+6,-3);
    \node [draw, scale=0.8] (cc) at (-0.25+6,-1.5) {};
    \node [draw, scale=0.8] (ccc) at (-0.8+6,-2.5) {};
    \node[below=1pt] at (ccc) {$p$};
    \node [draw, scale=0.8] (cccc) at (-0.3+6,-2.5) {};
    \node [draw, scale=0.8] (pcc) at (0.25+6,-1.5) {};
    \node [draw, scale=0.8] (pccc) at (0.8+6,-2.5) {};
    \node [draw, scale=0.8] (pcccc) at (0.3+6,-2.5) {};
    \node[below=1pt] at (pcccc) {$q$};
    \draw [-latex', opacity=0.35] (c) to (cc);
    \draw [-latex',  opacity=0.35] (cc) to (ccc);
    \draw [-latex',  opacity=0.35] (cc) to (cccc);
    \draw [-latex', opacity=0.35] (c) to (pcc);
    \draw [-latex',  opacity=0.35] (pcc) to (pccc);
    \draw [-latex',  opacity=0.35] (pcc) to (pcccc);
    
    \node [draw, circle, scale =0.7] (d) at (9,0) {$\exists x_4$};
    \draw [-latex'] (d) to (-1.4+9,-3);
    \draw [-latex'] (d) to (1.4+9,-3);
    \node [draw, scale=0.8] (dd) at (-0.25+9,-1.5) {};
    \node [draw, scale=0.8] (ddd) at (-0.8+9,-2.5) {};
    \node[below=1pt] at (ddd) {$p$};
    \node [draw, scale=0.8] (dddd) at (-0.3+9,-2.5) {};
    \node [draw, scale=0.8] (pdd) at (0.25+9,-1.5) {};
    \node [draw, scale=0.8] (pddd) at (0.8+9,-2.5) {};
    \node [draw, scale=0.8] (pdddd) at (0.3+9,-2.5) {};
    \node[below=1pt] at (pdddd) {$q$};
    \draw [-latex', opacity=0.35] (d) to (dd);
    \draw [-latex',  opacity=0.35] (dd) to (ddd);
    \draw [-latex',  opacity=0.35] (dd) to (dddd);
    \draw [-latex', opacity=0.35] (d) to (pdd);
    \draw [-latex',  opacity=0.35] (pdd) to (pddd);
    \draw [-latex',  opacity=0.35] (pdd) to (pdddd);	
    %%%%%%%
    \node [draw, fill=\FigColA!40!white, scale=0.8] at (-0.25+3,-1.5) {}; 
    \draw [thick, \FigColA](-0.25,-1.5)  ellipse (0.5 and 0.5);
    \draw [-latex', thick] (a) to (aa);\draw [-latex', thick] (b) to (bb);
    \draw [-latex', bend right =30 ,\FigColA, thick] (-0.25,-1.70) to (-0.25+3,-1.70);
    \draw [thick, \FigColA](0,0)  ellipse (0.5 and 0.5);
    \draw [-latex', bend right =30 ,\FigColA, thick] (0,-0.55) to (-0.5+3,-1.50);
    \end{scope}
%  \end{tikzpicture} 
%  \begin{tikzpicture}[xscale=1.1, yscale=0.7]
    \begin{scope}[yshift=-4cm]
      \node [circle, draw, scale =0.7] (a) at (0,0) {$\forall  x_1$}; 
    \node [text width=2.1cm] at (-1.25+0.05,-0.5) {\scriptsize \begin{tabular}{c}Side \\dependences\end{tabular}}; 
    \draw [-latex'] (a) to (-1.4,-3);
    \draw [-latex'] (a) to (1.4,-3);
    \node [draw, scale=0.8] (aa) at (-0.25,-1.5) {};
    \node [draw, scale=0.8] (aaa) at (-0.8,-2.5) {};
    \node[below=1pt] at (aaa) {$p$};
    \node [draw, scale=0.8] (aaaa) at (-0.3,-2.5) {};
    \node [draw, scale=0.8] (paa) at (0.25,-1.5) {};
    \node [draw, scale=0.8] (paaa) at (0.8,-2.5) {};
    \node [draw, scale=0.8] (paaaa) at (0.3,-2.5) {};
    \node[below=1pt] at (paaaa) {$q$};
    \draw [-latex', opacity=0.35] (a) to (aa);
    \draw [-latex', opacity=0.35] (aa) to (aaa);
    \draw [-latex',  opacity=0.35] (aa) to (aaaa);
    \draw [-latex', opacity=0.35] (a) to (paa);
    \draw [-latex', opacity=0.35] (paa) to (paaa);
    \draw [-latex',  opacity=0.35] (paa) to (paaaa);
    
    \node [scale =0.7, circle, draw] (b) at (3,0) {$\exists  x_2$};
    \draw [-latex'] (b) to (-1.4+3,-3);
    \draw [-latex'] (b) to (1.4+3,-3);
    \node [draw, scale=0.8] (bb) at (-0.25+3,-1.5) {};
    \node [draw, scale=0.8] (bbb) at (-0.8+3,-2.5) {};
    \node[below=1pt] at (bbb) {$p$};
    \node [draw, scale=0.8] (bbbb) at (-0.3+3,-2.5) {};
    \node [draw, scale=0.8] (pbb) at (0.25+3,-1.5) {};
    \node [draw, scale=0.8] (pbbb) at (0.8+3,-2.5) {};
    \node [draw, scale=0.8] (pbbbb) at (0.3+3,-2.5) {};
    \node[below=1pt] at (pbbbb) {$q$};
    \draw [-latex', opacity=0.35] (b) to (bb);
    \draw [-latex',  opacity=0.35] (bb) to (bbb);
    \draw [-latex',  opacity=0.35] (bb) to (bbbb);
    \draw [-latex', opacity=0.35] (b) to (pbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbbb);
    
    \node [circle,draw, scale =0.7] (c) at (6,0) {$\forall  x_3$}; 
    \draw [-latex'] (c) to (-1.4+6,-3);
    \draw [-latex'] (c) to (1.4+6,-3);
    \node [draw, scale=0.8] (cc) at (-0.25+6,-1.5) {};
    \node [draw, scale=0.8] (ccc) at (-0.8+6,-2.5) {};
    \node[below=1pt] at (ccc) {$p$};
    \node [draw, scale=0.8] (cccc) at (-0.3+6,-2.5) {};
    \node [draw, scale=0.8] (pcc) at (0.25+6,-1.5) {};
    \node [draw, scale=0.8] (pccc) at (0.8+6,-2.5) {};
    \node [draw, scale=0.8] (pcccc) at (0.3+6,-2.5) {};
    \node[below=1pt] at (pcccc) {$q$};
    \draw [-latex', opacity=0.35] (c) to (cc);
    \draw [-latex',  opacity=0.35] (cc) to (ccc);
    \draw [-latex',  opacity=0.35] (cc) to (cccc);
    \draw [-latex', opacity=0.35] (c) to (pcc);
    \draw [-latex',  opacity=0.35] (pcc) to (pccc);
    \draw [-latex',  opacity=0.35] (pcc) to (pcccc);
    
    \node [draw, circle, scale =0.7] (d) at (9,0) {$\exists  x_4$};
    \draw [-latex'] (d) to (-1.4+9,-3);
    \draw [-latex'] (d) to (1.4+9,-3);
    \node [draw, scale=0.8] (dd) at (-0.25+9,-1.5) {};
    \node [draw, scale=0.8] (ddd) at (-0.8+9,-2.5) {};
    \node[below=1pt] at (ddd) {$p$};
    \node [draw, scale=0.8] (dddd) at (-0.3+9,-2.5) {};
    \node [draw, scale=0.8] (pdd) at (0.25+9,-1.5) {};
    \node [draw, scale=0.8] (pddd) at (0.8+9,-2.5) {};
    \node [draw, scale=0.8] (pdddd) at (0.3+9,-2.5) {};
    \node[below=1pt] at (pdddd) {$q$};
    \draw [-latex', opacity=0.35] (d) to (dd);
    \draw [-latex',  opacity=0.35] (dd) to (ddd);
    \draw [-latex',  opacity=0.35] (dd) to (dddd);
    \draw [-latex', opacity=0.35] (d) to (pdd);
    \draw [-latex',  opacity=0.35] (pdd) to (pddd);
    \draw [-latex',  opacity=0.35] (pdd) to (pdddd);	
    %%%%%%%
    \node [draw, fill=\FigColA!40!white, scale=0.8] at (-0.25+3,-1.5) {}; \draw [thick, \FigColA](0.25,-1.5)  ellipse (0.5 and 0.5);
    \draw [-latex', thick] (a) to (paa);\draw [-latex', thick] (b) to (bb);
    \draw [-latex', bend right =30 ,\FigColA, thick] (0.25,-1.70) to (-0.25+3,-1.70);
    \end{scope}
  %\end{tikzpicture}
  %\begin{tikzpicture}[xscale=1.1, yscale=0.7]
    \begin{scope}[yshift=-8cm]
      \node [circle, draw, scale =0.7] (a) at (0,0) {$\forall x_1$}; 
    \node [text width=2.1cm] at (-1.25+0.05,-0.5) {\scriptsize \begin{tabular}{c}Future \\dependences\end{tabular}}; 
    \draw [-latex'] (a) to (-1.4,-3);
    \draw [-latex'] (a) to (1.4,-3);
    \node [draw, scale=0.8] (aa) at (-0.25,-1.5) {};
    \node [draw, scale=0.8] (aaa) at (-0.8,-2.5) {};
    \node[below=1pt] at (aaa) {$p$};
    \node [draw, scale=0.8] (aaaa) at (-0.3,-2.5) {};
    \node [draw, scale=0.8] (paa) at (0.25,-1.5) {};
    \node [draw, scale=0.8] (paaa) at (0.8,-2.5) {};
    \node [draw, scale=0.8] (paaaa) at (0.3,-2.5) {};
    \node[below=1pt] at (paaaa) {$q$};
    \draw [-latex', opacity=0.35] (a) to (aa);
    \draw [-latex', opacity=0.35] (aa) to (aaa);
    \draw [-latex',  opacity=0.35] (aa) to (aaaa);
    \draw [-latex', opacity=0.35] (a) to (paa);
    \draw [-latex', opacity=0.35] (paa) to (paaa);
    \draw [-latex',  opacity=0.35] (paa) to (paaaa);
    
    \node [scale =0.7, circle, draw, fill=\FigColA!40!white, ] (b) at (3,0) {$\exists x_2$};
    \draw [-latex'] (b) to (-1.4+3,-3);
    \draw [-latex'] (b) to (1.4+3,-3);
    \node [draw, scale=0.8] (bb) at (-0.25+3,-1.5) {};
    \node [draw, scale=0.8] (bbb) at (-0.8+3,-2.5) {};
    \node[below=1pt] at (bbb) {$p$};
    \node [draw, scale=0.8] (bbbb) at (-0.3+3,-2.5) {};
    \node [draw, scale=0.8] (pbb) at (0.25+3,-1.5) {};
    \node [draw, scale=0.8] (pbbb) at (0.8+3,-2.5) {};
    \node [draw, scale=0.8] (pbbbb) at (0.3+3,-2.5) {};
    \node[below=1pt] at (pbbbb) {$q$};
    \draw [-latex', opacity=0.35] (b) to (bb);
    \draw [-latex',  opacity=0.35] (bb) to (bbb);
    \draw [-latex',  opacity=0.35] (bb) to (bbbb);
    \draw [-latex', opacity=0.35] (b) to (pbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbbb);
    
    \node [circle,draw, scale =0.7] (c) at (6,0) {$\forall x_3$}; 
    \draw [-latex'] (c) to (-1.4+6,-3);
    \draw [-latex'] (c) to (1.4+6,-3);
    \node [draw, scale=0.8] (cc) at (-0.25+6,-1.5) {};
    \node [draw, scale=0.8] (ccc) at (-0.8+6,-2.5) {};
    \node[below=1pt] at (ccc) {$p$};
    \node [draw, scale=0.8] (cccc) at (-0.3+6,-2.5) {};
    \node [draw, scale=0.8] (pcc) at (0.25+6,-1.5) {};
    \node [draw, scale=0.8] (pccc) at (0.8+6,-2.5) {};
    \node [draw, scale=0.8] (pcccc) at (0.3+6,-2.5) {};
    \node[below=1pt] at (pcccc) {$q$};
    \draw [-latex', opacity=0.35] (c) to (cc);
    \draw [-latex',  opacity=0.35] (cc) to (ccc);
    \draw [-latex',  opacity=0.35] (cc) to (cccc);
    \draw [-latex', opacity=0.35] (c) to (pcc);
    \draw [-latex',  opacity=0.35] (pcc) to (pccc);
    \draw [-latex',  opacity=0.35] (pcc) to (pcccc);
    
    \node [draw, circle, scale =0.7] (d) at (9,0) {$\exists x_4$};
    \draw [-latex'] (d) to (-1.4+9,-3);
    \draw [-latex'] (d) to (1.4+9,-3);
    \node [draw, scale=0.8] (dd) at (-0.25+9,-1.5) {};
    \node [draw, scale=0.8] (ddd) at (-0.8+9,-2.5) {};
    \node[below=1pt] at (ddd) {$p$};
    \node [draw, scale=0.8] (dddd) at (-0.3+9,-2.5) {};
    \node [draw, scale=0.8] (pdd) at (0.25+9,-1.5) {};
    \node [draw, scale=0.8] (pddd) at (0.8+9,-2.5) {};
    \node [draw, scale=0.8] (pdddd) at (0.3+9,-2.5) {};
    \node[below=1pt] at (pdddd) {$q$};
    \draw [-latex', opacity=0.35] (d) to (dd);
    \draw [-latex',  opacity=0.35] (dd) to (ddd);
    \draw [-latex',  opacity=0.35] (dd) to (dddd);
    \draw [-latex', opacity=0.35] (d) to (pdd);
    \draw [-latex',  opacity=0.35] (pdd) to (pddd);
    \draw [-latex',  opacity=0.35] (pdd) to (pdddd);	
    %%%%%%%
    \draw [thick, \FigColA](-0.25,-1.5)  ellipse (0.5 and 0.5);
    \draw [-latex', thick] (a) to (aa);
    \draw [-latex', bend right =30 ,\FigColA, thick] (-0.25,-1.70) to (-0.35+3,-0.50);
    \end{scope}
    %  \end{tikzpicture}
%   \\[+5pt]
%  \begin{tikzpicture}[xscale=1.1, yscale=0.7]
    \begin{scope}[yshift=-12cm,xshift=0cm]
      \path[use as bounding box] (11,-3.2);
      \draw [thick, \FigColB, rounded corners] (-1.6,0.6) rectangle (10.6,-3.3);
    %
    \node [fill=white] at (-1.25-0.2,-1) {\scriptsize \begin{tabular}{@{}c@{}}Adding \\active goals\\ on current\\ history.\end{tabular}}; 
    \node [fill=white, text=\FigColB] at (10.6,-1) {\small \begin{tabular}{@{}c@{}}Only in\\ Section~\ref{se::AddingAction}.\end{tabular}};
    %%
    %%
    %%
    \node [circle, draw, scale =0.7] (a) at (0,0) {$\forall  x_1$}; 
    
    \draw [-latex'] (a) to (-1.4,-3);
    \draw [-latex'] (a) to (1.4,-3);
    \node [draw, scale=0.8] (aa) at (-0.25,-1.5) {};
    \node [draw, scale=0.8] (aaa) at (-0.8,-2.5) {};
    \node[below=1pt] at (aaa) {$p$};
    \node [draw, scale=0.8] (aaaa) at (-0.3,-2.5) {};
    \node [draw, scale=0.8] (paa) at (0.25,-1.5) {};
    \node [draw, scale=0.8] (paaa) at (0.8,-2.5) {};
    \node [draw, scale=0.8] (paaaa) at (0.3,-2.5) {};
    \node[below=1pt] at (paaaa) {$q$};
    \draw [-latex', opacity=0.35] (a) to (aa);
    \draw [-latex', opacity=0.35] (aa) to (aaa);
    \draw [-latex',  opacity=0.35] (aa) to (aaaa);
    \draw [-latex', opacity=0.35] (a) to (paa);
    \draw [-latex', opacity=0.35] (paa) to (paaa);
    \draw [-latex',  opacity=0.35] (paa) to (paaaa);
    
    \node [scale =0.7, circle, draw] (b) at (3,0) {$\exists x_2$};
    \draw [-latex'] (b) to (-1.4+3,-3);
    \draw [-latex'] (b) to (1.4+3,-3);
    \node [draw, scale=0.8] (bb) at (-0.25+3,-1.5) {};
    \node [draw, scale=0.8] (bbb) at (-0.8+3,-2.5) {};
    \node[below=1pt] at (bbb) {$p$};
    \node [draw, scale=0.8] (bbbb) at (-0.3+3,-2.5) {};
    \node [draw, scale=0.8] (pbb) at (0.25+3,-1.5) {};
    \node [draw, scale=0.8] (pbbb) at (0.8+3,-2.5) {};
    \node [draw, scale=0.8] (pbbbb) at (0.3+3,-2.5) {};
    \node[below=1pt] at (pbbbb) {$q$};
    \draw [-latex', opacity=0.35] (b) to (bb);
    \draw [-latex',  opacity=0.35] (bb) to (bbb);
    \draw [-latex',  opacity=0.35] (bb) to (bbbb);
    \draw [-latex', opacity=0.35] (b) to (pbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbb);
    \draw [-latex',  opacity=0.35] (pbb) to (pbbbb);
    
    \node [circle,draw, scale =0.7] (c) at (6,0) {$\forall x_3$}; 
    \draw [-latex'] (c) to (-1.4+6,-3);
    \draw [-latex'] (c) to (1.4+6,-3);
    \node [draw, scale=0.8] (cc) at (-0.25+6,-1.5) {};
    \node [draw, scale=0.8] (ccc) at (-0.8+6,-2.5) {};
    \node[below=1pt] at (ccc) {$p$};
    \node [draw, scale=0.8] (cccc) at (-0.3+6,-2.5) {};
    \node [draw, scale=0.8] (pcc) at (0.25+6,-1.5) {};
    \node [draw, scale=0.8] (pccc) at (0.8+6,-2.5) {};
    \node [draw, scale=0.8] (pcccc) at (0.3+6,-2.5) {};
    \node[below=1pt] at (pcccc) {$q$};
    \draw [-latex', opacity=0.35] (c) to (cc);
    \draw [-latex',  opacity=0.35] (cc) to (ccc);
    \draw [-latex',  opacity=0.35] (cc) to (cccc);
    \draw [-latex', opacity=0.35] (c) to (pcc);
    \draw [-latex',  opacity=0.35] (pcc) to (pccc);
    \draw [-latex',  opacity=0.35] (pcc) to (pcccc);
    
    \node [draw, circle, scale =0.7] (d) at (9,0) {$\exists x_4$};
    \draw [-latex'] (d) to (-1.4+9,-3);
    \draw [-latex'] (d) to (1.4+9,-3);
    \node [draw, scale=0.8] (dd) at (-0.25+9,-1.5) {};
    \node [draw, scale=0.8] (ddd) at (-0.8+9,-2.5) {};
    \node[below=1pt] at (ddd) {$p$};
    \node [draw, scale=0.8] (dddd) at (-0.3+9,-2.5) {};
    \node [draw, scale=0.8] (pdd) at (0.25+9,-1.5) {};
    \node [draw, scale=0.8] (pddd) at (0.8+9,-2.5) {};
    \node [draw, scale=0.8] (pdddd) at (0.3+9,-2.5) {};
    \node[below=1pt] at (pdddd) {$q$};
    \draw [-latex', opacity=0.35] (d) to (dd);
    \draw [-latex',  opacity=0.35] (dd) to (ddd);
    \draw [-latex',  opacity=0.35] (dd) to (dddd);
    \draw [-latex', opacity=0.35] (d) to (pdd);
    \draw [-latex',  opacity=0.35] (pdd) to (pddd);
    \draw [-latex',  opacity=0.35] (pdd) to (pdddd);	
    %%%%%%%
    \node [draw, fill=\FigColA!40!white, scale=0.8] at (-0.25+3,-1.5) {};
    \draw [thick, \FigColA](0,0)  ellipse (0.5 and 0.5);
    \draw [-latex', bend right =30 ,\FigColA, thick] (0,-0.55) to (-0.5+3,-1.5);
    \draw [thick, \FigColA](0+6,0)  ellipse (0.5 and 0.5);
    \draw [-latex', bend left =30 ,\FigColA, thick] (0+6,-0.55) to (-0.05+3,-1.5);
    \draw [thick, \FigColA] (d)  ellipse (0.5 and 0.5);
    \draw [thick, -latex', \FigColA] (9,-0.55) to[out=-90,in=-90] (-0.25+3,-1.75);
    \end{scope}
  \end{tikzpicture}
  %\vspace*{-10mm}
  \caption{The different kinds of dependences.}
  \label{FigureLayoutFourkindOfInfluence}
\end{figure}

